Reactive Locomotion Decision-Making and Robust Motion Planning for Real-Time Perturbation Recovery

In this paper, we examine the problem of push recovery for bipedal robot locomotion and present a reactive decision-making and robust planning framework for locomotion resilient to external perturbations. Rejecting perturbations is an essential capability of bipedal robots and has been widely studied in the locomotion literature. However, adversarial disturbances and aggressive turning can lead to negative lateral step width (i.e., crossed-leg scenarios) with unstable motions and self-collision risks. These motion planning problems are computationally difficult and have not been explored under a hierarchically integrated task and motion planning method. We explore a planning and decision-making framework that closely ties linear-temporal-logic-based reactive synthesis with trajectory optimization incorporating the robot's full-body dynamics, kinematics, and leg collision avoidance constraints. Between the high-level discrete symbolic decision-making and the low-level continuous motion planning, behavior trees serve as a reactive interface to handle perturbations occurring at any time of the locomotion process. Our experimental results show the efficacy of our method in generating resilient recovery behaviors in response to diverse perturbations from any direction with bounded magnitudes.

==> removed.tex <==

% \textbf{Leg crossing is a special motion worth highlighting in this study. However, to make the planning method complete, it might be helpful to frame the planner in a general way, i.e., design recovery strategies for both leg crossing and non-leg-crossing situations.}

\section{Introduction}

AI planning methods have been receiving more interest as the complexity of task planning problems increase.

% \noindent\textbf{Why do we need symbolic planning and high-level decision-making for dynamic legged locomotion? What is the limit of few existing methods (less formal, very heuristic)?}


% \Ye{For the intro paragraphs, find a decent balance between AI planning and dynamic locomotion? such that reviewers from either side will appreciate this work. If locomotion folks read this work, will they use our AI method for their robots? If symbolic planning folks read this work, will they believe the locomotion problem is a meaningful application of BTs?}

% \noindent\textbf{How to provide formal safety/stability guarantee in the presence of terrain disturbances?}
% In this paper, we mainly consider the situation of flat ground. We don't have a clear formal guarantee for terrain yet. I added the terrain disturbance as a further work in the discussion section.

%(This is more implementation) To formulate the LTL problem, the robot action is the foot placement and center-of-mass (CoM) state of a reduced-order locomotion model and the environment is modeled as an adversarial external disturbance.

% However, the symbolic planning only accounts for disturbance at discrete keyframe instances, which imposes a strong environmental disturbance assumptions. To deal with disturbances that can happen anytime, we utilize the BTs as a reactive, and scalable, discrete-to-continuous intermediary with trajectory optimization to locally change the motion to a safe state in a robust Riemannian manifold. Highly constrained gait motions are generated using kinodynamic-aware trajectory optimization and consolidated into a gait library for step transitions that avoid self collision.

% In particular, our method contains multiple novel components in: (i) proposing a high-level symbolic task planner that is commonly under-explored in the field of locomotion to make discrete locomotion decisions; (ii) employing behavior trees as the middle-level execution layer to handle external perturbations that can occur at any continuous time during the locomotion excursion; and (iii) designing a full-body-dynamics-aware TO, particularly in addressing a bipedal walking leg-crossing problem that is subject to leg collision constraints, which need more investigations in the push recovery literature.
% Although more complex, real-world perturbations such as terrain uncertainty and visual perception disturbance are not explicitly modeled in this paper. Instead, the CoM perturbations are representative of these issues and allows us to explore the fundamental principles of resilient decision-making and planning for robust locomotion. This helps clarify the handling of more complex perturbations during tasks in the future. 
 
%The reason that we want to use behavior tree is that: 1. behavior tree is modular and flexible and reusable and reactive. It is great option for online planning that react to external disturbance. In what scenario does BT help, why is it a must? Why is it better than finite state machine? How can the automaton be translated to BT, is it difficult? (performance, metric, quantify, success rate convergence?)

% For instance, in the presence of a lateral perturbation under gait specific constraints, the system could require a leg crossing motion as shown in Fig.~\ref{fig:vision}. The robot would have to not only plan its next foot placement but also consider avoiding leg self-collision during the motion. 

% We address this problem by incorporating the kinodynamic-aware trajectory optimization (TO) for successful step transitions, to bridge the gap between high-level, reduced-order, keyframe-based task planning and low-level, joint-space motion planning.


% \Ye{in this BT paragraph, we should explain why LTL synthesis is not enough. This is because it only handles discrete-level decision (i.e., keyframe-level decision). Perturbations at non-apex states can not be addressed by LTL but BT. }

\subsection{Robot Model} % Combine this section with Appendix A in some way.

% Talk about the robot model
As shown in Figure \ref{fig:vision}, we uses the Prismatic Inverted Pendulum Model (PIPM) for high level symbolic planning. The model decouples the CoM motion in sagittal and lateral, which provides flexibility for keyframe decision making. Using dynamic balance of moments, the difference between the moments acting on the contact foot and the net inertial and gravitational moments, is zero. Therefore, for the single contact scenario, the PIPM dynamics is:
$$
-\bm{p}_{foot} \times \bm{f}_r + \bm{p}_{CoM} \times (\bm{f}_{CoM} + m\bm{g}) + \bm{\tau}_{CoM} = 0
$$
The $\bm{f}_{CoM}$ and $\bm{\tau}_{CoM}$ are CoM inertial force and torque, and $\bm{f}_r$ is the ground reaction force on the support leg.

% Talk about the disturbance rejection, put it in related works.
Keeping balance during walking is the most prominent safety requirement for humanoid robot locomotion. The goal of the framework is to find a policy that is guaranteed to provide feasible recovery strategy to keep the robot from falling under the disturbances. Some disturbance can trip the robot because it triggers a leg crossing scenario that have the risk of self-collision. So the framework helps to provide a guarantee of successful recovery motion under modeled environment disturbance.

\section{Problem Formulation}

% Talks about the goal of the framework.
Robot is most capable with the form factor of a human. [] Humanoid robots are able to traverse in the world built for human and operate tasks similar to what human can do.
Bipedal system, however, is an inherently unstable and under-actuated system requiring active control to stay balance. Error sources coming from sensor noise, inaccurate modeling, or terrain perturbations dramatically affect the performance of task execution and even fail the task. Therefore, we aim to address the research problem of disturbance rejection for legged locomotion system. To this end, we propose a framework that formally guarantee the execution of locomotion task. 

% Introduce how we formulate the problem and what methods are used.
We consider the ubiquitous scenario of bipedal walking where external disturbances induce state jumps. 

Given the nature of disturbance can happen anytime in a normal walking cycle, we model the disturbance as a 
Considering a disturbance happens on the system, the goal of the problem is to find a robust motion that recovery from a disturbed state to a steady state 

The goal of the task planner is to create a robust keyframe decision maker. The decision maker chooses keyframe transitions to complete the locomotion task in the next 2 steps. The formulation of the planner synthesis problem comprises 3 components: the robot model, the assumptions on bounded (aka, admissible) environment, and the desired system specification. 

\subsection{State Estimation}

We use state estimation to fuse onboard sensor data (IMU and joint encoder), detect the environment disturbance, and estimate the impacted system state. The state estimation uses kinematics chain to compute the swing leg jacobian, which maps the leg joint rotation rate into the pelvis frame velocity:
$$v_{wf} = v_{wp} + v_{pf} = J_{wf} \dot{q}_{floating joint} + J_{pf} \dot{q}_{stance}$$ 
$J_{pf}$ is the jacobian from the pelvis frame (root of the kinematics chain) to the foot frame. We assume the stance foot does not slide on the ground or treadmill belt. The ground is stationary, even on treadmill, we assume the world frame is attached to the non-moving part of the treadmill. So we have $v_{wf} = 0$. Thus the CoM velocity is $v_{wp} = -J_{pf} \dot{q}_{stance}$.

We estimate the keyframe state based on the timing. We use the phase variable $\tau$ to represent how far the current state has moved along the gait trajectory. We assume each gait has a fixed step time, $t = 0.4$. So the phase variable $\tau = 0.5$ represent apex time, at which time the state is keyframe state.

One of the key advantage of BT is its reactivity. While gait is executed under one subtree, if a significant environment change happens, the BT tree would automatically choose another available solution gait to handle the perturbation and induce seamless transition between gaits under perturb.


\subsection{LTL}

The success of the reactive synthesis problem relies on the critical step: 1. The abstraction of the infinite-state system into a equivalent finite state model such that any discrete plan generated by the discrete planner can be implemented by the continuous controller, provided that the evolution of the controller state satisfy the system locomotion dynamics. 2. synthesis of a discrete planner, represented by a finite state automaton, that ensures the correctness of the discrete plan. \cite{Receding-Horizon-Temporal-Logic} % [13]

To formally guarantee that the safety specifications are met, we use General Reactivity of Rank 1 (GR(1)), a fragment of Linear Temporal Logic (LTL). GR(1) allows us to design temporal logic formulas ($\varphi$) with atomic propositions (AP ($\varphi$)) that can either be \textsf{True} ($\varphi \vee \neg\varphi$) or \textsf{False} ($\neg$\textsf{True}). With negation ($\neg$) and disjunction ($\vee$) one can also define the following operators: conjunction ($\wedge$), implication ($\Rightarrow$), and equivalence ($\Leftrightarrow$). There also exist temporal operators ``next" ($\bigcirc$), ``until" ($\mathcal{U}$), ``eventually" ($\Diamond$), and ``always" ($\square$). Further details of GR(1) can be found in \cite{gr1}. {\color{red}(Rewrite)}

% \begin{equation}
% \begin{aligned}
% &\square \, (s_f \in s_c \wedge v(s_c)) \\
% &\square \, ((s,s') \in \mathcal{T}) \\
% &\square \, (p(s') \in [c_l, c_r]) 
% \end{aligned}
% \end{equation}

%We try to minimize the damage caused by the disturbance, and we consider position displacement is a form of damage. On treadmill system, going over the bound is dangerous and terrain is void and has a huge velocity discrepancy. Finally, if the keyframe state is $K_{ss}$, it stays.

\subsection{BT}

Every sub-tree of a BT can be treated as a standalone entity that represents a certain action or a task. BTs are equipped with control-flow nodes to capture various conditional, or sequential sub-tree executions, hence making BTs an appropriate formalism for reactive controllers. \cite{Maximally-satisfying-LTL} % [5]

It also automatically monitors the execution status of the task plan. Any low-level action failure would automatically trigger an update of high-level task abstraction and further trigger a re-planning procedure if necessary. \cite{Lan2019AutonomousTP} % [4]

BTs are built using sub-tree blocks in a hierarchical fashion, subsuming thus multiple levels of abstraction and allowing to easily replace an abstract action/task node with a concrete action/task implementation. \cite{unified-behavior-tree} % [6]


\subsection{TO}

The motion planning problem is modelled as a trajectory optimization problem. We discretize the Cassie trajectory, and transcribe the states and control into a Non-Linear Program (NLP). Consider the following NLP problem:

% $$
% X^* = \argmin_{X} \sum L_i(X_i)
% $$
% $$
% s.t. \; C^l_j \leq C_j(X_j) \leq C^u_j \\
% $$
% $$
% X^l \leq X \leq X^u
% $$
% Where $X$ represents the system states and control, $L_i(X_i)$ is the running cost along the current trajectory. Also $C_j(X_j)$ and $X$ should follow the system constraint formulated as inequality constraints.

\section{Results}
% Our experimentation sought to answer the following primary questions: (1) Can safe behaviors be effectively generated for any time point at both a symbolic and geometric planning level? (2) How does including symbolic planning enable more effective and flexible multi-step gait strategies?
